Algebraic Multigrid Methods For Virtual Element Discretizations: A Numerical Study

We investigate the performance of algebraic multigrid methods for the solution of the linear system of equations arising from a Virtual Element discretization. We provide numerical experiments on very general polygonal meshes for a model elliptic problem with and without highly heterogeneous diffusion coefficients and we draw conclusions regarding the efficacy of the method.

==> comput_time.tex <==
\subsection{Computational efficiency}
\label{computational_times}

We compare the performance of several direct and iterative solvers and  
convergence is decided by the decrease of the residual norm relative to the norm of right hand side obtained with the direct solver SuperLU\_DIST, \texttt{rtol} reported in each Table.
%With mesh voro$_{10}$, CG without preconditioning requires more than $10000$ iterations to reach convergence.
%With meshes voro$_9$ and voro$_{10}$, UMFPACK fails due to an \emph{out of memory} error.


%
%%%%%%%
\input{full_tables}


%%%% Hexa jumping \rho


\begin{landscape}
	%%%% Aggregated hexagons - jumping coeffcients
	
	\begin{table}
		\vspace{2.cm} 
		\centering
		\caption{Performance of direct and iterative solvers on the the hexagonal meshes hexa$_2$, hexa$_4$, hexa$_6$, hexa$_8$ and hexa$_{10}$ shown in Table~\ref{tab:mesh-hexa}
						with jumping coefficients $\rho$ as described in Section~\ref{sec:lowest-random}. 
				We report the time for setup and solving for both direct and iterative solvers. 
				From top to bottom, concerning the number of parts which Voronoi meshes are partitioned into, we consider $L = 64, 256, 1024$, respectively.
						Convergence is decided by the decrease of the residual norm relative to the norm of right hand side obtained with the direct solver SuperLU\_DIST, \texttt{rtol}.
			%		Both SuperLU and UMFPACK fails on a-horse$_5$ and a-horse$_6$ due to an \emph{out of memory} error.
		}
		\label{tab:k1-hexa-jump}
		\small
		\begin{tabular}{c
				S[table-format=7.0]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
				S[table-format=1.{\roundPrecision}]
			}
			\toprule
			{Mesh}       & {Dof}   & {c-GAMG}& {a-GAMG}& {BoomerAMG}& {ML}&{SuperLU}&{UMFPACK}& {MUMPS}&{SuperLu DIST}&  {Pastix}\\
			\midrule
			$L = 64$     &         &         &         &         &        &        &        &         &        & \\
			\midrule	
			hexa$_{8}$   &  80604  & 0.91213& 0.60452 & 0.26308 &   0.306  &   4.3881 &  1.7315 & 2.3106 &  1.6881 & 1.8712  \\
			hexa$_{8}$   &  321204 & 3.9874 &  2.9554 & 1.0634  &   1.6689 &  39.8    & 10.098  & 15.643 & 10.841  & 12.499 \\
			hexa$_{8}$   &  721804 & 8.3183 & 6.0131  & 2.6356  &   3.449  & 188.9    & 35.454  & 52.661 & 30.718  & 36.769 \\
			hexa$_{8}$   & 1282404 & 15.22  & 11.719  & 4.5659  &   6.2838 & 445.33   &  *      & 124.48 & 72.509  & 84.145 \\
			hexa$_{8}$   & 2003004 &  *     & *       & 7.1908  &  12.95   & 907.64   &  *      & 231.43 & 138.22  & 161.01 \\
			\midrule
			$L = 256$    &         &        &         &         &         &        &        &        &         & \\
			\midrule  
			hexa$_{8}$   &  80604  & 1.1396 &  1.5927 & 0.27117 &  1.1405 & 4.3793 & 3.1394&  2.3095&  1.6736 &  1.8742 \\
			hexa$_{8}$   &  321204 & 5.5811 &  7.9401 & 1.101   &  5.5657 & 39.85  &  14.702 & 15.746 & 10.779  &  12.279 \\
			hexa$_{8}$   &  721804 & 13.857  &  17.538 & 2.5346  &  12.916 & 189.11 & 36.378& 52.616& 31.157  & 36.772 \\
			hexa$_{8}$   & 1282404 & 27.385 & 38.986 & 4.2508  &  30.537 & 445.29 &  *     & 124.58& 72.302  & 84.136 \\
			hexa$_{8}$   & 2003004 & 32.243 & 40.656  & 6.8684  &  36.397 & 907.12 &  *     & 232.23& 137.11  & 161.23\\
			\midrule
			$L = 1024$   &         &        &         &         &         &        &        &        &         &       \\
			\midrule
			hexa$_{8}$   &  80604 & 5.0487 &  14.688 & 0.28678 &  16.315 & 4.3622 &  5.8249&  2.3098&  1.6676 & 1.8786  \\
			hexa$_{8}$   &  321204 & 14.182 &  33.694 & 1.2879  &  32.948 & 39.667 & 23.247 & 15.696 & 10.846  & 12.432 \\
			hexa$_{8}$   &  721804 & 56.76  &  89.818 & 2.608   &  93.934 & 189.55 & 218.18 & 52.661 & 31.021  & 36.804 \\
			hexa$_{8}$   & 1282404 & 65.313 & 135.07  & 4.7267  & 119.62  & 445.16 &  *     & 124.6  & 72.557  & 83.913 \\
			hexa$_{8}$   & 2003004 & 136.96 & 293.3   & 6.9779  & 326.04  & 906.21 &  *     & 231.67 & 137.36  & 160.99 \\
			\bottomrule
		\end{tabular}
	\end{table}
\end{landscape}	
	
	
	\begin{landscape}
		%%%% Aggregated hexagons - jumping coeffcients
		
		\begin{table}
			\vspace{2.cm} 
			\centering
			\caption{Performance of direct and iterative solvers on the Voronoi meshes voro$_5$--voro$_{10}$ shown in Table~\ref{tab:k1-voro}
			 partitioned with METIS, %approximation order $k = 1$,\
				with jumping coefficients $\rho$ as described in Section~\ref{sec:lowest-random}. 
				We report the time for setup and solving for both direct and iterative solvers. 
				From top to bottom, concerning the number of parts which Voronoi meshes are partitioned into, we consider $L = 64, 256, 1024$, respectively.
			}
			\label{tab:k1-voro-jump}
			\small
			\begin{tabular}{c
					S[table-format=7.0]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
					S[table-format=1.{\roundPrecision}]
				}
				\toprule
				{Mesh}       & {Dof}   & {c-GAMG}& {a-GAMG}& {BoomerAMG}& {ML}&{SuperLU}&{UMFPACK}& {MUMPS}&{SuperLu DIST}&  {Pastix}\\
				\midrule
				$L = 64$     &         &         &         &         &        &        &        &         &        & \\
				\midrule
	%			voro$_3$  &   20007 &   0.23919&  0.25732&  0.10895&  0.13239 &   0.23658& 0.13599 &   0.25138 & 0.23264& 0.22645  \\
	%			voro$_4$  &   40011 &  0.52486 &  0.44939 & 0.23189 &  0.30533 &   0.6672 & 0.3344 &  0.5939 & 0.5522& 0.50317 \\
				voro$_5$  &   80007 & 1.1242  &  0.93814 &0.45836 & 0.5768 &   1.7456  &  0.69415  &  0.9249&  1.1542 &   1.0735 \\
				voro$_6$  &  160028 &  2.4742  &  1.948  & 0.97389 & 1.1381   &  4.7006   & 1.8806 &  2.114& 2.3426& 2.3281 \\
				voro$_7$  &  320020 &  4.9139 & 3.8165& 2.1262 & 2.5677    & 13.965 & 5.149  & 4.5343& 5.6466   & 5.0226\\
				voro$_8$  &  640035 & 11.446  & 9.9439   & 4.1607& 6.2731   & 44.107 & 15.385    & 11.396 & 13.214 & 11.738\\
				voro$_9$  & 1280053 & 22.953 & 18.485  & 9.4007& 12.282   & 141.96   &  *           & 27.486  & 30.713& 24.234\\
			    voro$_{10}$ & 2560065 & 56.681  & 38.991  & 20.469 & 29.222     & 440.35  &  *           & 69.928 & 79.336  & 68.286\\
				\midrule
				$L = 256$    &         &        &         &         &         &        &        &        &         & \\
				\midrule  
	%			voro$_3$     &   20007 & 0.61384 &  0.80825& 0.095413&  0.82717  & 0.22203 & 0.1465 &   0.20897 &  0.2357&0.23317 \\
	%			voro$_4$     &   40011 &  1.0748 &  1.0095  &   0.21166 &  0.84182 & 0.5914 &  0.31841 &  0.46142 & 0.50776 &  0.51628 \\
				voro$_5$     &   80007 & 3.4119 & 2.7438   & 0.42168 &  2.9882 & 1.6566   & 0.80297 &  0.96547 & 1.16  & 1.1609\\
				voro$_6$     &  160028 &  7.899 & 6.6927   & 0.92577&  6.9114  &  4.7524 & 2.0617 &  2.2502 & 2.4988&  2.3292 \\
				voro$_7$     &  320020 &  17.728 & 12.949   & 1.9803 &12.307    & 15.251   & 6.0724   & 4.7861   & 5.5394 & 5.2971\\
				voro$_8$     &  640035 & 31.062  & 21.867   & 4.0734 &19.958   & 44.929   & 15.798  & 11.106 & 13.835 & 12.573 \\
				voro$_9$     & 1280053 & 81.295 & 68.561   & 8.6757&59.375   & 141.91    &  *            & 27.182  & 30.348  & 25.432\\
				voro$_{10}$ & 2560065 & 200.05 & 153.04     & 19.306 &122.13   & 434.59     &  *           & 68.077 & 78.262  & 70.057\\
				\midrule
				$L = 1024$   &         &        &         &         &         &        &        &        &         &       \\
				\midrule
	%			voro$_3$     &   20007   & 7.5051 &   19.614 & 0.093928&  39.306 &  0.22929&  0.19838&  0.19466&  0.2367 &    0.25418 \\
		%		voro$_4$     &   40011   & 15.481 &  28.51 & 0.20548&  65.728 & 0.67522  & 0.34193& 0.42387& 0.55088  &   0.51623\\
				voro$_5$     &   80007   & 17.681  &  31.527 & 0.42791 &  54.97& 1.8051 &  0.85573  &0.91368 & 1.0881  &   1.2039 \\
				voro$_6$     &  160028  & 54.848 &  61.183& 0.90888 & 99.723 & 5.1732   & 2.1392 & 2.1111 & 2.4783 &   2.4435 \\
				voro$_7$     &  320020  & 69.004&  71.455  & 1.8899& 117.25& 14.902  & 7.0265& 5.0092 & 5.4639  &   5.3808 \\
				voro$_8$     &  640035  & 185 & 161.8  & 4.0643&  263.58 & 45.08  & 22.43  &10.934 & 13.229  &  12.831 \\
				voro$_9$     & 1280053 & 379.29 & 313.6 &  8.6875 & 435.63 & 138.42   &  *           & 27.262 &  31.028  & 26.664 \\
				voro$_{10}$ & 2560065 & 655.66& 481.54  & 19.199 & 539.27  & 434.54  &  *           &  68.618 & 79.845  & 71.502 \\
				\bottomrule
			\end{tabular}
		\end{table}
	\end{landscape}	

%
%
%%\input{new_numerical}
%


